The Users Aren't Alright: Dangerous Mental Illness Behaviors and Recommendations

In this paper, we argue that recommendation systems are in a unique position to propagate dangerous and cruel behaviors to people with mental illnesses.

==> oldwriting.tex <==
% \section{Introduction}

% Recommendation systems are a driving force in the technological ecosystem that individuals interact with in their daily lives, from community engagement on social media to fulfilling material needs from e-commerce sites. The relationship between users and recommendation systems is generally mutually beneficial as users are presented with content that they need while the systems obtain data in the form of the user's interactions to further create more robust recommendations. However, what happens when these recommendation systems are presented with dangerous behavioral interactions from users? A recommendation system has no concept of what is ``safe" or ``harmful" and thus can not assess the interaction behaviors being introduced, and therefore takes in and propagates harmful behaviors to users with similar inferred needs. While many users would be able to assess if a recommendation is ``harmful" to them and act accordingly, users with high-risk mental health disorders may not recognize these recommendations as ``harmful" or do but it encourages their high-risk behaviors. We focus on mental health specifically, as dangerous behaviors in this domain are harder to detect and even more challenging to mitigate.

% In theory, recommendation systems will internalize users' harmful mental health behaviors and propagate them to other users, does this actually happen in the wild? We found several examples from live recommendation systems that do just that. 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.7\linewidth]{Figures/amazonsuicide.png}
%     \caption{Amazon Recommendation for Sodium Nitrite}
%     \label{fig:amazon_suicide}
% \end{figure}
% In this first example showcased in Figure \ref{fig:amazon_suicide}, we present the Amazon recommendation for the item Sodium Nitrite, a substance commonly known to be used by individuals to end their lives. The item recommended with this substance is Tagamet, an over-the-counter acid reducer and heartburn relief medicine. When a person ingests Sodium Nitrite their body will naturally try and purge the chemical, but if taken with Tagamet the body will be less likely to try and purge the toxin, increasing the likelihood of death. The showcased recommendation is in essence providing a suicide method as a one-click add-to-cart solution where the individual does not even need to have background knowledge about the suicide cocktail.  
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figures/amazon caffine.png}
%     \caption{Amazon Recommendation Accompanying Caffeine Pills}
%     \label{fig:amazon_caffine}
% \end{figure}
% While the previous example is very obvious in its harmfulness, as it can directly facilitate someone taking their own life, we also found some more subtle examples. Figure \ref{fig:amazon_caffine} depicts the recommendations associated with a caffeine supplement which are commonly used by people struggling with eating disorders. The accompanying recommendations are for an appetite suppressant and a weight loss supplement. The combination of products does seem logical but when a person with an eating disorder encounters these recommendations is it encouraging a harmful behavior. Further, dietary supplements are not reviewed by the FDA before they go to market \cite{FDA} and there is no information provided on how the recommended supplements may interact with each other.

% These examples are only two of many that illustrate the propagation of users' harmful mental health behaviors in recommendation systems. While the examples we have provided are specifically Amazon, the problem can be found in other recommendation systems. A study conducted on YouTube and Twitter examined the contagion effect of the blue whale challenge, which encourages users to self-harm and kill themselves \cite{khasawneh2020examining}. Both of the aforementioned platforms rely heavily on recommendations for distributing content to users. While harmful behaviors and the products or content glorifying them have always been present, recommendation systems are currently spreading and exposing at-risk users to these products and content without them ever needing to go looking. 

% Fueled by these examples and previous literature on technologies' influence on at-risk populations, it is our position that recommendation systems are in a unique position to propagate dangerous behaviors and have profound impacts on individuals and that researchers from academia and industry should consider the safety of at-risk users who interact with recommendation systems and be held accountable for the impact recommendations can have on users. In taking this position, there are several questions that come to mind:
% \begin{enumerate}
%     \item What would it mean for a recommender system to consider users' safety?
%     \item Where would intervention for users' safety fit in recommendation systems?
%     \item How will researchers be held accountable? 
% \end{enumerate}
% As such in the remainder of this work, we dive into related work and consider on the above questions, as well as possible ways to begin addressing them.

% \section{Related Work}

% \subsection{Contagion Effect}
% Blue Whale: Examining the self-harm and suicide contagion effects of the Blue Whale Challenge on YouTube and Twitter: qualitative study

% suicide: Suicide conversations on Instagram™: contagion or caring?

% Social Emotion: Digital Emotion Contagion

% \subsection{Algorithmic Cruelty}
% In short, recommended content can lead to what is now termed as “algorithmic cruelty” by the popular press and academic research, connecting to research around algorithmic impacts after breakups [8] and traumatic life events [6]. Prior work has focused on how specific technology-mediated reflections, like those that bring up memories, can be challenging for individuals to manage [6,8]. Other work has focused on how moderation negatively impacts peoples’ access to supportive communities in times of distress [4,5]. It is now clear through multiple public reports that this “double-edged sword” is playing out in real recommendation systems that are damaging to peoples’ well-being, as Instagram has received scrutiny for its impact on teens [1]. 

% 1. Charles Riley Business CNN. Instagram says it’s working on body image issue after report details “toxic” effect on teen girls. CNN. Retrieved July 13, 2022 from https://www.cnn.com/2021/09/15/tech/instagram-teen-girls/index.html
% 4.	Jessica L Feuston and Anne Marie Piper. 2019. Everyday Experiences: Small Stories and Mental Illness on Instagram. In Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems (CHI ’19), 1–14. https://doi.org/10.1145/3290605.3300495
% 5.	Jessica L. Feuston, Alex S. Taylor, and Anne Marie Piper. 2020. Conformity of Eating Disorders through Content Moderation. Proceedings of the ACM on Human-Computer Interaction 4, CSCW1: 1–28. https://doi.org/10.1145/3392845
% 6.	Caitlin Lustig, Artie Konrad, and Jed R. Brubaker. 2022. Designing for the Bittersweet: Improving Sensitive Experiences with Recommender Systems. In CHI Conference on Human Factors in Computing Systems, 1–18. https://doi.org/10.1145/3491102.3502049
% 8.	Anthony T. Pinter, Jialun Aaron Jiang, Katie Z. Gach, Melanie M. Sidwell, James E. Dykes, and Jed R. Brubaker. 2019. “Am I Never Going to Be Free of All This Crap?”: Upsetting Encounters with Algorithmically Curated Content About Ex-Partners. Proceedings of the ACM on Human-Computer Interaction 3, CSCW: 1–23. https://doi.org/10.1145/3359172

%Questions such as these are also not unique, this question is often postulated in ethics research. Trying to answer this question can very quickly devolve into the blame game and so shifting the focus to how accountability should be enforced, regardless of who is accountable, is just as important.

%Human-centered centered computing research has started to be integrated into several fields, for example, human-centered machine learning. As different fields begin to embrace the human-centered nature of technology the gravity of the effect that different systems have on users becomes more clear, thus equivocating the consequences to the how can be better understood. With the rise in human-centered focused research, some mechanisms for accountability have already started being implemented. 

%Another major component of recommendation is the presentation of content, most recommendations consist of a description and an image making even how the recommendation has displayed a factor in users' safety. Both words and images have the potential of conveying complex emotional components that could be provoking for at-risk users. For example, Facebook will recommend old photos from a user's timeline which for some users will bring back cherished memories, but for others, it is possible that it is dredging up painful memories due to the loss of loved ones or traumatic events. While the images and description proved for a product or content are not controlled by the recommendation system, the propensity for that item to be recommended is. Thus, by considering what content or products should ethically be allowed to have associated recommendations or have recommendations attached, a recommendation system can safeguard users from harmful triggers or stigmas associated with their at-risk status.

%There are, however, existing intervention strategies for recommendation systems, one such example is parental controls on social media sites. These controls allow parents to control what content their children are being exposed to and in theory, could be used by at-risk users to control if they would be exposed to harmful recommendations. Flagging or indicating that a user does not want to see specific content is also common in social media recommendation systems but is often hard to get to or does not seem to have an effect from the user's perspective [CITE? this is a spoiler from our study soooooo maybe can use]. While interface or setting interventions may be possible, studies would need to be conducted to establish if at-risk users would utilize such features and how those settings should be integrated.


